The Feeling of Success: Does Touch Sensing Help Predict Grasp Outcomes?

A successful grasp requires careful balancing of the contact forces. Deducing whether a particular grasp will be successful from indirect measurements, such as vision, is therefore quite challenging, and direct sensing of contacts through touch sensing provides an appealing avenue toward more successful and consistent robotic grasping. However, in order to fully evaluate the value of touch sensing for grasp outcome prediction, we must understand how touch sensing can influence outcome prediction accuracy when combined with other modalities. Doing so using conventional model-based techniques is exceptionally difficult. In this work, we investigate the question of whether touch sensing aids in predicting grasp outcomes within a multimodal sensing framework that combines vision and touch. To that end, we collected more than 9,000 grasping trials using a two-finger gripper equipped with GelSight high-resolution tactile sensors on each finger, and evaluated visuo-tactile deep neural network models to directly predict grasp outcomes from either modality individually, and from both modalities together. Our experimental results indicate that incorporating tactile readings substantially improve grasping performance.

==> 7_discussion.tex <==
Although the proposed approach allowed us to study the importance of tactile sensing for robotic grasping, this method by itself is not necessarily an ideal solution for practical robotic grasping.
The learned model provides a rejection mechanism that evaluates the outcome of a grasp after the grasp is actually performed (but before liftoff).
As such, based on the quality of the proposing mechanism, convergence to an acceptable grasp might take an arbitrarily high number of grasp attempts.
In our experiments, we used a basic random search to propose new grasp location, which was sufficient to address the main experimental hypothesis of our work.
Although in most of the experiments a good solution would typically be accepted within 3 or 4 grasps, some trials took substantially longer, with one trial requiring 45 grasps before lifting the object successfully.
Moreover, our approach does not explicitly consider any post-liftoff event, such as slipping, hence not making full use of the interactive nature of tactile information for grasping.
Future work should aim to overcome these two limitations by proposing visuo-tactile solutions that are practical for real-world robot grasping. 


